Approximating the Gaussian Multiple Description Rate Region Under Symmetric Distortion Constraints

We consider multiple description coding for the Gaussian source with K descriptions under the symmetric mean squared error distortion constraints, and provide an approximate characterization of the rate region. We show that the rate region can be sandwiched between two polytopes, between which the gap can be upper bounded by constants dependent on the number of descriptions, but independent of the exact distortion constraints. Underlying this result is an exact characterization of the lossless multi-level diversity source coding problem: a lossless counterpart of the MD problem. This connection provides a polytopic template for the inner and outer bounds to the rate region. In order to establish the outer bound, we generalize Ozarow's technique to introduce a strategic expansion of the original probability space by more than one random variables. For the symmetric rate case with any number of descriptions, we show that the gap between the upper bound and the lower bound for the individual description rate is no larger than 0.92 bit. The results developed in this work also suggest the "separation" approach of combining successive refinement quantization and lossless multi-level diversity coding is a competitive one, since it is only a constant away from the optimum. The results are further extended to general sources under the mean squared error distortion measure, where a similar but looser bound on the gap holds.

==> Conclusion.tex <==
\section{Conclusion}
\label{sec:con}

We provide approximate characterizations of the individual-description R-D function, as well as the achievable rate region, for the Gaussian MD problem under symmetric distortion constraints. This is done by combining two inter-connected parts: the derivation of a novel outer bound, and careful analysis of achievability schemes to generate inner bounds for easy comparison with the outer bound. The outer bound alone, or the inner bound alone, will not be able to provide this results, and particular care has to be taken in order to make them compatible. A result in a similar vein was recently obtained by Etkin {\em et al.} \cite{Etkin:07} for Gaussian interference channel.

The new lower bound is obtained by generalizing Ozarow's well-known technique, and expand the probability space of the original problem by more than one random variables with special structure among them. This technique appears to be promising, and we expect to see its application in other difficult multi-terminal information-theoretic communication problems. 

The multi-level diversity coding problem, which can be understood as a lossless counterpart of the MD problem, shed tremendous light on the geometric structure of the MD rate-distortion region. We use the lossless MLD coding rate region as a polytopic template for both inner and outer bounds for the MD rate-distortion region. With the increasing complexity of a source coding problem being considered in information theory literature, we expect the complexity of its lossless counterpart to increase as well, and the difficulty of the corresponding lossless problem becomes an increasingly dominant component of the overall problem. In this context, our work can be understood as the first attempt to make explicit connection between the lossless source coding problem and its lossy counterpart. It is worth noting in multi-terminal channel coding problems, several well-known recent works can be understood as using deterministic models, for example, the network coding results in \cite{Yeung:00}, and the deterministic wireless relay channel model in  \cite{Avestimehr:07}. There exists a philosophical connection between the approach taken in this work and the ``one-bit" approximation result for the Gaussian interference channel in \cite{Etkin:07}, as well as the approximate capacity result for the Gaussian relay network  \cite{Avestimehr:08}. In \cite{Avestimehr:08}, an approximate characterization was motivated by the insight obtained in studying deterministic relay networks \cite{Avestimehr:07}, which has an analogous role as the lossless multi-level diversity coding problem in our work. In both cases, the connection provides useful insight to the coding scheme and outer bounding proof technique. We expect in the near future connection between the lossless (deterministic) model and their lossy (non-deterministic) counterpart to be made on other information theoretic problems, and the approach of using the former as a guideline in treating the latter to be a fruitful path. 
